Advances on CNN-based super-resolution of Sentinel-2 images

Thanks to their temporal-spatial coverage and free access, Sentinel-2 images are very interesting for the community. However, a relatively coarse spatial resolution, compared to that of state-of-the-art commercial products, motivates the study of super-resolution techniques to mitigate such a limitation. Specifically, thirtheen bands are sensed simultaneously but at different spatial resolutions: 10, 20, and 60 meters depending on the spectral location. Here, building upon our previous convolutional neural network (CNN) based method, we propose an improved CNN solution to super-resolve the 20-m resolution bands benefiting spatial details conveyed by the accompanying 10-m spectral bands.

==> Advances on CNN-based super-resolution of Sentinel-2 imageS/preambol.tex <==
% correct bad hyphenation here
\hyphenation{op-tical net-works semi-conduc-tor}
\usepackage{spconf,amsmath,epsfig}

\usepackage{spconf,amsmath,graphicx}
\usepackage{subfig}
\usepackage{color,soul}
\usepackage{epstopdf}
\usepackage{tikz}
\usepackage{balance}
\usepackage{url}
\usepackage{multirow,hhline}
\usepackage{placeins}
\usepackage{wasysym}
\usepackage{amssymb}

\usepackage[nomessages]{fp}% http://ctan.org/pkg/fp
\captionsetup{belowskip = -5pt}

% My commands
\renewcommand{\aa}[1]{{\bf \textcolor{blue}{#1}}}
\newcommand{\bb}[1]{{\bf \textcolor{red}{#1}}}
\newcommand{\point}{\item \vspace{-2mm}}
%\newcommand{\Dlambda}{{\bf D}$_\lambda$}
%\newcommand{\Desse}{{\bf D}$_{\rm S}$}
%\newcommand{\ru}{\rule{0pt}{7pt}}
\newcommand{\abstracttext}{\textbf}

\newcommand{\bx}{\mathbf{x}}
\newcommand{\by}{\mathbf{y}}
\newcommand{\bw}{\mathbf{w}}
\newcommand{\bz}{\mathbf{z}}
\newcommand{\bZ}{\mathbf{Z}}
\newcommand{\bbb}{\mathbf{b}}
\newcommand{\bu}{\mathbf{u}}
\newcommand{\hx}{\hat{\mathbf{x}}}
\newcommand{\hy}{\hat{\mathbf{y}}}
\newcommand{\hM}{\hat{M}}
\newcommand{\tM}{\widetilde{M}}
\newcommand{\tx}{\widetilde{\mathbf{x}}}
\newcommand{\xH}{\widetilde{\mathbf{x}}_{\rm H}}
\newcommand{\zH}{\mathbf{z}_{\rm H}}


\newcommand{\PL}{\mathbf{PL}}
\newcommand{\M}{\mathbf{M}} % original res. MS
\newcommand{\PAN}{\mathbf{P}} % original res. PAN
\newcommand{\F}{\mathbf{F}} % original res. PANSHARPENED / FUSED
\newcommand{\R}{\mathbf{R}} % original res. REFERENCE

\newcommand{\labsty}[1]{{\scriptsize #1}}

\DeclareMathOperator{\BN}{BN}
\DeclareMathOperator{\E}{E}
\DeclareMathOperator{\Q}{Q}
\DeclareMathOperator{\Var}{Var}
\DeclareMathOperator{\SAM}{SAM}
\DeclareMathOperator{\RMSE}{RMSE}
\DeclareMathOperator{\ERGAS}{ERGAS}
\DeclareMathOperator{\QNR}{QNR}
\DeclareMathOperator{\DS}{D_S}
\DeclareMathOperator{\DL}{D_{\lambda}}
\DeclareMathOperator{\DSast}{D_S^\ast}
\DeclareMathOperator{\DLast}{D_{\lambda}^\ast}

\newcommand{\PNN}[3]{{D#1-K#2-F#3}}

\newcommand{\image}{\pgfuseimage}

\newcommand{\figpath}{./Figures/}
\newcommand{\pngBIG}{./PNG/Result_Paper_Entire/}
\newcommand{\pngDET}{./PNG/Result_Paper_Mazzini/}
\newcommand{\pngFULL}{./PNG/Result_Paper_Mazzini_Full/}
\definecolor{colPeppe}{rgb}{0.7, 0.2, 0.15}
\newcommand{\peppe}[1]{{\color{colPeppe} #1}}

\definecolor{colSico}{rgb}{0.9, 0.5, 0.1}
\newcommand{\sico}[1]{{\color{colSico}\textbf{#1}  }}

%%%%%%%%IMAGE & TABLES%%%%%%%%%%%%%

\pgfdeclareimage[width=0.9\textwidth]{net2}{\figpath flowchart.pdf}

\newcommand{\widBIG}{3.2cm}
\newcommand{\widDET}{2.4cm}

\pgfdeclareimage[width=\widBIG]{Bx}{\pngBIG 004_RGBDR_RGB.png}
\pgfdeclareimage[width=\widBIG]{Bz}{\pngBIG 004_RGBD_RGB.png}
\pgfdeclareimage[width=\widBIG]{Br}{\pngBIG 004_RGB_RGB.png}
\pgfdeclareimage[width=\widBIG]{Bhpf}{\pngBIG 004_RGB__HPF_RGB.png}
\pgfdeclareimage[width=\widBIG]{Bfive}{\pngBIG 004_RGB_PANIGARSS_RGB.png}
\pgfdeclareimage[width=\widBIG]{Bprop}{\pngBIG 004_RGB_PANS5HBTY_RGB.png}

\pgfdeclareimage[width=\widDET]{Dx}{\pngDET 004_RGBDR_RGB.png}
\pgfdeclareimage[width=\widDET]{Dz}{\pngDET 004_RGBD_RGB.png}
\pgfdeclareimage[width=\widDET]{Dr}{\pngDET 004_RGB_RGB.png}
\pgfdeclareimage[width=\widDET]{Dhpf}{\pngDET 004_RGB__HPF_RGB.png}
\pgfdeclareimage[width=\widDET]{Dfive}{\pngDET 004_RGB_PANIGARSS_RGB.png}
\pgfdeclareimage[width=\widDET]{Dprop}{\pngDET 004_RGB_PANS5HBTY_RGB.png}

\pgfdeclareimage[width=\widDET]{Fx}{\pngFULL 004_RGB_bicubic_RGB.png}
\pgfdeclareimage[width=\widDET]{Fz}{\pngFULL 004_RGB_RGB.png}
\pgfdeclareimage[width=\widDET]{Fhpf}{\pngFULL 004_RGB__HPF_band_RGB.png}
\pgfdeclareimage[width=\widDET]{Ffive}{\pngFULL 004_RGB_PANIGARSS_RGB.png}
\pgfdeclareimage[width=\widDET]{Fprop}{\pngFULL 004_RGB_PANS5HBTY_RGB.png}



%%%%% TABLE REDIFINITION %%%%%%%%%%%%
\newcommand{\best}[1]{{\bf \textcolor{blue}{#1}}}
\newcommand{\bbst}[1]{{\bf \textcolor{blue}{#1}}}
\newcommand{\bstc}[1]{{\bf \textcolor{blue}{#1}}}
\newcommand{\bstp}[1]{{\bf \textcolor{red}{#1}}}
\newcommand{\ru}{\rule{0mm}{3mm}}

\newcommand{\propA}{L1}
\newcommand{\propB}{L1-RL}
\newcommand{\propC}{L1-RL-self}
\newcommand{\propD}{L1-RL-FT}

\newcommand{\propE}{Baseline+ (IK)}
\newcommand{\propF}{Baseline+ (IK)/self}
\newcommand{\propX}{L1 (cross-sensor)}
\newcommand{\propG}{L1-RL (cross-sensor)}
\newcommand{\propH}{L1-RL (cross-sensor)-FT}

\newcommand{\Dlambda}{{\bf D}$_\lambda$}
\newcommand{\Desse}{{\bf D}$_S$}


